Resource Allocation of Industry 4.0 Micro-Service Applications across Serverless Fog Federation

The Industry 4.0 revolution has been made possible via AI-based applications (e.g., for automation and maintenance) deployed on the serverless edge (aka fog) computing platforms at the industrial sites -- where the data is generated. Nevertheless, fulfilling the fault-intolerant and real-time constraints of Industry 4.0 applications on resource-limited fog systems in remote industrial sites (e.g., offshore oil fields) that are uncertain, disaster-prone, and have no cloud access is challenging. It is this challenge that our research aims at addressing. We consider the inelastic nature of the fog systems, software architecture of the industrial applications (micro-service-based versus monolithic), and scarcity of human experts in remote sites. To enable cloud-like elasticity, our approach is to dynamically and seamlessly (i.e., without human intervention) federate nearby fog systems. Then, we develop serverless resource allocation solutions that are cognizant of the applications' software architecture, their latency requirements, and distributed nature of the underlying infrastructure. We propose methods to seamlessly and optimally partition micro-service-based application across the federated fog. Our experimental evaluation express that not only the elasticity is overcome in a serverless manner, but also our developed application partitioning method can serve around 20% more tasks on-time than the existing methods in the literature.

==> Sources/conclsn.tex <==
\section{Conclusion and Future Works}\label{concl}
Transitioning to Industry 4.0, particularly at remote sites, entails the ability to handle modern micro-service workflows with strict latency constraints near data sources and in a serverless manner. The problem, however, is that under emergency situation, near-data fog computing systems quickly become oversubscribed and cannot handle the situation effectively. To overcome this challenge, we developed a platform for serverless industrial fog federation that is aware of the software architecture of the industrial applications and the characteristics (uncertainties) of the fog federation. The proposed platform operates within the gateways representing each fog system and makes fog federation serverless via hiding the topological complexities of the federation from the user's perspective. The platform's goal is achieved via two modules: the first one models each micro-service application as a DAG and tries to optimally partition it to subgraphs that can make use of the federation. Then, the second module, which is for resource allocation, maps the partitions across the fog federation via considering both computation and communication latencies. Evaluation results show the efficacy of the proposed platform, particularly under oversubscribed situations, where it brings about $\sim$15\%---18\% higher deadline meet rate in compare to other widely-used partitioning and resource allocation methods. Moreover, we noted that proposed solution for the federation is scalable and can dynamically handle different number of fogs in the federation. 

In the future, we plan to handle industrial use cases such as industrial monitoring operation (\eg drilling), that have to run uninterruptedly, across the federation. For that purpose, we are going to develop live service migration across the federation. \textcolor{blue}{In order to effectively manage industrial applications, it is imperative to support task priorities, such as urgent tasks with hard deadlines and best-effort tasks with soft deadlines (\cite{hujo2021toward,nouinou2023decision}). One complication is that some tasks of a certain industrial application can be considered as urgent, whereas, other tasks of the same application expose best-effort behavior. For the example of object detection application, the tasks used for fire detection (\cite{zhao2022fire}) are deemed urgent with hard deadlines, whereas, tasks for detecting employees' faces are best-effort and with lower priority. Demonstrating the feasibility of fog federation and partitioning micro-service workflows across it, one future avenue of this research can focus on the task characteristics and priorities across the fog federation.} Another avenue for the future study will be performing partitioning in a more granular manner---within each micro-service. For instance, for ML-based micro-services, we can perform pre-processing on the source fog and neural network processing on another fog in the federation.



==> Sources/intro.tex <==
\section{Introduction}\label{intro}
dsfs ddfsd 
\subsection{Overview and Motivation}
% The advancement of IoT technologies with smart applications drives the wheel of the Industry 4.0 \cite{lu2019oil} revolution. Various sensors, actuators, and smart IoT devices are deployed in different industries (\eg manufacturing, food processing, oil \& gas, sustainable energy) that control the operational technology platform \cite{bramantyo2022data,titu2020merging} to achieve automation, production efficiency, and safety. Accordingly, sensors utilized in industrial operations frequently produce tons of data every day \cite{daily2017predictive}. The oil and gas industry is an example of generating enormous amounts of sensor data and the necessity for processing close to the data source. For instance, a typical offshore oil rig produces 1 to 2 TB of data daily \cite{sof2}. Most of this data is fed to Industry 4.0 smart applications (\eg machine learning, report generation, automation) to make latency-sensitive decisions, thereby, improving the energy efficiency, production, and safety measures. For example, applications like workplace air quality estimation \cite{kristiani2021implementation} for workers' safety utilize environmental sensors that measure the quality (\ie the existence of harmful particles in the air) of breathable air in the surrounding of the workplace. Hence, the air quality estimation must be fast to avoid potential hazards to human workers.  
Industrial systems are rapidly shifting from human-controlled processes towards closed-loop serverless control systems (\cite{8637768, pei2020towards,mahmoud2019architecture,9144772}) that process various types of applications to manage industrial operations autonomously. Particularly at remote sites, such as offshore oil and gas fields (\cite{hussain2022iot}), space stations (\cite{aume2022trackink}), and submarines and underwater robots (ROVs) (\cite{kabanov2022marine}), the Industry 4.0 paradigm shift demands systems to serverlessly process emerging data-driven and latency-sensitive applications under harsh operational environment where there is limited/no access to the cloud services, and human resources are scarce and not computer literate. Realizing these systems mandates addressing challenging research questions to enable robust, latency-aware, and serverless processing of the applications on alternative computing platforms (\cite{wang2019big,8291112, cai2019iot}) operating atop low-latency wireless communication systems (\cite{al2019scalable}).


To overcome the lack of reliable access to cloud servers, making use of the fog computing systems (a.k.a. cloudlets) (\cite{mattia2023p2pfaas}) in remote industrial sites has become a common practice. %On the contrary, managing and maintenance of the fog system for executing latency sensitive Industry 4.0 applications raises the demand for having a serverless \cite{} platform that augment the separation of application deployment from configuring the run-time servers. 
Nonetheless, these fog systems inherently suffer from the lack of elasticity (\cite{nguyen2020elasticfog}) and fail to handle workload spikes often occur due to unpredictable disasters that the remote industrial sites are prone to (\cite{chiou2022robot}). An exemplar use case is a remote (offshore) oil field where, upon detecting an oil spill, the following coordinated activities must be processed within a short period of time: (A) Drones must be dispatched for more granular investigation; (B) Emergency teams must be notified; and (C) High-end simulations must be conducted for purposes like predicting the oil spill expansion direction, and staff evacuation. 

To establish an Industry 4.0 system in a remote site that is robust against such unpredictabilities, we explore the challenging idea of augmenting the processing capability of the local fog via dynamically federating it with nearby fog systems (\eg mobile datacenters (\cite{thayananthan2015big})), thereby, providing cloud-like serverless elasticity for Industry 4.0 applications. This challenge stems from the fact that modern industrial applications are often cloud-native, and are not originally designed to reap the benefits of wirelessly-connected autonomous fogs. \emph{There is an infrastructural gap to adapt these applications to the federated fog environment, and this gap is what this research aims at filling}. More specifically, the challenge is how to establish the notion of serverless such that the applications can seamlessly take advantage of the dynamically formed federated fog system? To overcome this challenge, we need to deal with two aspects of the federated environments: 

\noindent\textit{(a) Characteristics of the federated fog environment}:
The federated fog environment is prone to the uncertainties stem from the unreliable communication between fog system, and heterogeneous computing across them. Both of these uncertainties can potentially affect the latency constraint of Industry 4.0 applications across the federation. Failure to dealing with these uncertainties so can potentially hurt the robustness of remote site instead of helping it (\cite{salehi2016stochastic}).

\noindent\textit{(b) Characteristics of Industry 4.0 applications}: Most of the current Industry 4.0 applications function based on  Machine Learning (ML-based) and typically follow the micro-service-based software architecture (\cite{jwo2022data,aberle2022microservice}) where a workflow of micro-services (\cite{dragoni2017microservices}) have to be completed within a deadline. There are also legacy applications with monolithic architecture that are inflexible and have to be allocated in an atomic manner (\ie cannot be partitioned into modules) (\cite{calderon2018integration}). Unlike monolithic applications, micro-services are composed of several independent services that can be deployed separately. For instance, as depicted in figure \ref{fig:workflowMicro}, a ``fire safety" application can include a workflow of micro-services that includes services for capturing video surveillance data, pre-processing the captured video, noise removal, feature extraction, fire detection, location mapping, alert generation, and expansion prediction. 





% In the remote offshore industry, several services (\eg data acquisition, alert generation, object tracking) are critical for emergencies (\eg accidents, disasters) where various activities need to be performed synchronously. The situation can worsen when any unwanted emergency brings many more computational activities that need to be completed within limited time frames. In this case, our motivation is the smart Oil and Gas industry that has been facing various disasters and catastrophes (\eg the deepwater horizon (2010)\cite{srinivasan2010many}, usumacinta jack-up disaster (2007) \cite{hanlon2013usumacinta}, mumbai high north disaster (2005) \cite{daley2013mumbai}, the ocean ranger disaster (1982) \cite{heising1989ocean} ) due to complex fault intolerant industrial processes in exploration, drilling, and production operations. Therefore, remote offshore industries need latency-aware computing support \cite{deng2021intelligent} that can not be feasible with typical cloud data centers due to the remote locations of the industrial operation sites. The current solution utilizes fluctuating satellite communication \cite{cricelli2022market} for sending data to mainland cloud data centers reducing the quality of service (QoS) and increasing the industrial safety risk. Hence, the high-level challenge is the lack of computational resources to support oversubscribed situations in remote industries.

\begin{figure}[h!]
	\centering	
	\includegraphics[scale=0.62]{Figures/workflowMicroservicesFireSafety_1.pdf}
	\caption{Workflow of micro-services needed for the ``fire detection'' application. The application needs to seamlessly make use of federated fog to complete on time and prevent any potential damage.\label{fig:workflowMicro}}
\end{figure}

In sum, an ideal platform for remote sites should be: (i) serverless in the sense that it can seamlessly supply resources for both monolithic and micro-service applications across the federation; and (ii) robust against the network and computing uncertainties such that it can fulfill the  latency (deadline) constraints of the applications.% The Industry 4.0 platform must be aware of such a constraint and execute the applications to fulfill it.


\subsection{Problem Statement and Contributions}
As depicted in Figure \ref{fig:layerFog}, for the use case of remote smart oil fields, a federated fog computing can be formed via wireless communication between nearby fog servers. Considering each fog system $i$ as a node (gateway) $G_i$ and the wireless links between them as edges, we can conceptually model the federated fog in form of a graph that the federated fog platform operates upon. It is noteworthy that each fog system is configured with a different set of resources, \ie there is a heterogeneity across fog systems. In this system, uncertainty exists in both the communication and computation times of the same task running across the federation. Accordingly, to meet the latency constraints (deadline) of the applications, the federated fog platform should be cognizant of these communication and computing heterogeneity and uncertainties, in addition to the applications' characteristics and latency requirements. 

\begin{figure}[h!]
	\centering	
	\includegraphics[scale=0.60]{Figures/introFogLayer.pdf}
	\caption{A multi-layer view of the serverless fog federation infrastructure in the context of offshore smart oil and gas industry. Micro-service and monolithic Industry 4.0 applications seamlessly run across the federated fog systems by means of a platform, deployed on each gateway ($G_i$) representing a fog system. \label{fig:layerFog}}
\end{figure}

Considering the heterogeneity across fog systems, in our prior work~(\cite{hussain2020analyzing}), we explored and identified the stochastic execution behavior of several Industry 4.0 applications across various type of machines. In another study~(\cite{hussain2019federated}), we investigated resource allocation strategies for the monolithic applications across the fog federations. 
Nonetheless, many real-world operational processes are carried out by means of applications with a workflow (Directed Acyclic Graph---DAG) of micro-services, where each micro-service is an independent entity that communicates its output data as the input to the next micro-service in the graph. Development and deployment of such applications on the federated fog entails the user's involvement in the topological and uncertainty details of the underlying infrastructure to ensure that the whole application is complete within its deadline. To establish the notion of serverless, the federated fog platform has to transparently take care of these details and allocate the application such that application's deadline is met.  

Micro-service DAGs offer the opportunity to perform the allocation at the micro-service level. That is, the platform can partition the workflow graph into subgraphs and allocate them across the federation. In this case, for a given workflow topology, and specific federation uncertainties, the two following questions have to be addressed: (1) How to partition the micro-service workflows, so that its deadline can be met? (2) How to allocate computing resources to the partitioned micro-services across fog federation, so that it has the highest likelihood of meeting its deadline?

To address these questions, we propose a load-balancing approach within the federated fog platform that is aware of both the application's software architecture, its deadline, and the underlying execution platform's characteristics. As a result, it enables cloud-like serverless behavior via dynamically and seamlessly allocating the applications across the federation. %our approach consists of two stages: 1) understanding the software architecture of the receiving applications and 2) allocating fog computing resources to micro-services for on-time execution completion. 
In summary, this paper makes the following contributions:
\begin{itemize}
    \item Developing a probabilistic method (called \textit{ProPar}) to optimally partition micro-service workflows across the fog federation in a transparent and serverless manner.%partitioning method that is aware of the underlying software architecture of Industry 4.0 applications.
    
    \item Developing a resource allocation method based on the Bayesian statistics that is cognizant of the application deadline and efficiently assigns partitioned workflows across the federation.% using serverless technology. 
    
    \item Evaluating and analyzing the partitioning and the resource allocation methods across the fog federation for Industry 4.0 applications.
\end{itemize}

The outcomes of this research lays the foundation upon which solution architects and industry experts can focus only on the business logic of their applications--either micro-service-based or monolithic--and leave the allocation details of their applications and handling the demand surge to the serverless fog federation platform. The rest of the paper is organized in the following manner. Section~\ref{relatedwork} presents related works as background studies. Section~\ref{sysModel} represents the system model. Section~\ref{partitioning} states the partitioning method of micro-service workflow across fog federation, whereas section~\ref{resourceAllocation} represents the resource allocation method for Industry 4.0 application. Section~\ref{result} demonstrates experimental setup, baseline techniques, and experimental results. Finally, section~\ref{concl} concludes the paper with some future avenues for exploration.

==> Sources/partitionHeuristic.tex <==
\section{Partitioning Micro-service Application Workflows}\label{partitioning}
%Maintaining latency constraints of a smart application comprising multiple micro-services depends on underlying software architecture and mapping of computational resources. For example, executing a micro-service application into a single fog system may not be possible or may not maintain its deadline constraint. On the other hand, a monolithic application can not be partitioned and can be considered an application with a single micro-service. For micro-service software architecture, partitioning the application into multiple partitions and allocating them across fog federation can increase the likelihood of its completion within the latency constraint. Furthermore, allocating appropriate computational resources to the partitioned micro-services also ensures the completion of the whole application workflow. 

\begin{figure}[h!]
	\centering	
	\includegraphics[scale=0.55]{Figures/partitioning_technique7.pdf}
	\caption{Flowchart of the ProPart workflow partitioning method. The output of this method is a partitioned workflow that is submitted to the resource allocation module, which is shown as the end step (with dashed lines) in this flowchart.\label{fig:partitionTech}}
\end{figure}  

%As such, our proposed solution consists of two stages. They are workflow partitioning and resource allocation.A detailed explanation of the partitioning stage is provided in the following subsections respectively.

%\subsection{Workflow partitioning} 

The main objective of the partitioning method is to partition a micro-service workflow application in a way that the application can meet its deadline. For that purpose, we need to measure the likelihood of on-time completion for workflow graph $\omega$, denoted $P(\omega)$, on a fog system. This requires knowing the probability of workflow completion before its deadline. To know the workflow deadline, we sum up the deadlines of its micro-services, \ie $ \delta_\omega = \Sigma_{i=1}^n m_i^\delta$. To learn the workflow completion, denoted $D_\omega$, we need to convolve the computational latency distributions of the micro-services in the critical path of $\omega$ that can be performed based on Equation~\ref{eq:convolve}. 
\begin{equation}\label{eq:convolve}
D_\omega = m_1^d \circledast m_2^d \circledast ....\circledast m_n^d    
\end{equation}

% to measure the probability of success for the entire workflow $\omega$
Using the completion time distribution ($D_\omega$), the probability of on-time completion for $\omega$ is the portion of $D_\omega$ that occurs before $\delta_\omega$ which is measured based on Equation~\ref{eq:prob}.

\begin{equation}\label{eq:prob}
P(\omega) =\mathbb P(D_\omega \leq \delta_\omega)
\end{equation}

Leveraging this theory, we can present our workflow partitioning method, called Probabilistic Partitioning (\textit{ProPart}). The flowchart of ProPart, shown in Figure~\ref{fig:partitionTech}, shows the steps to partition workflow $\omega$. In the first step, we assume executing the entire workflow on the receiving (local) fog system without any partitioning and calculate $P(\omega)$. The value of $P(\omega)$ is decisive on partitioning the workflow across the fog federation or executing it locally---on the receiving fog system---without partitioning it. To make this decision, the value of $P(\omega)$ is compared against a user-define value $\alpha$ (see Figure~\ref{fig:partitionTech}) that serves as a threshold determining how aggressively the user wants to take advantage of the federation. The lower values of $\alpha$ expresses the user tendency to execute $\omega$ locally and vice versa. In the extreme case, the user can forbid using the federation via choosing $\alpha=0$.
%COMMENT: INTERESTING EXPERIMENTS CAN BE DONE ON HE VALUE OF ALPHA AND TELL PEOPLE WHEN IT IS GOOD TO USE THE FEDERATION...
In our implementation, the value of $\alpha$ is adjustable, however, in the evaluation part, we consider $\alpha=50\%$. 

In the event that the likelihood of completing workflow $\omega$ is lower than $\alpha$, the graph partitioning operation has to be carried out. Finding the optimal number of partitions is an NP-complete problem (\cite{ccatalyurek2023more}), therefore, we develop a method based on the idea of divide and conquer (\cite{zhou2023qaoa}) to recursively find the most efficient way of partitioning $\omega$. The bare bones of the method is shown in the flowchart of Figure~\ref{fig:partitionTech}. At every step of this method, the graph is partitioned to two subgraphs, and for each subgraph the likelihood of success across the federation is calculated based on Equation~\ref{eq:prob}. The process continues until either the likelihood of success for at least one of the subgraphs is lower than or equal the parent graph, or the subgraphs have only one vertex (node). The former case implies that partitioning the graph does not improve the chance of success, hence, we roll-back to the parent graph and consider that subgraph as the appropriate partition that can be allocated to the fog federation. In the latter case, however, the graph cannot be partitioned any further and inevitably must be submitted for the resource allocator module.

To perform graph partitioning, we use the min-cut algorithm (\cite{lakhan2022deep}) that partitions workflow $\omega$ into two sub-graphs $i$ and $j$ based on the max-flow min-cut theorem (\cite{lochbihler2022mechanized}). The theorem states that the maximum flow (\eg amount of data) that can be transferred from a certain vertex (\eg micro-service) to another one is determined by the smallest bottleneck in the graph. Hence, to partition the workflow graph into sub-graphs, the min-cut algorithm finds the minimum number of edges that, if removed, the graph is partitioned to subgraphs. %Assuming that all the edges are equally significant, the algorithm removes the minimum edges to split the micro-service graph to two sub-graphs. 

According to Flowchart of Figure~\ref{fig:partitionTech}, at each iteration of the method, the partitions (subgraphs) resulted from the min-cut are estimated for their chances of success (meeting their deadlines) across the fog federation using Equations~\ref{eq:convolve} and~\ref{eq:prob}. If the likelihood of on-time completion of the partitioned graph is less than its parent graph (\ie $P(i) \leq P(\omega)$ or $P(j) \leq P(\omega)$), we consider the parent graph ($\omega$) as the optimal choice for allocation. In the next step, for each created partition, the resource allocation method is invoked (the last box in the flowchart). In the event that the partition's chance of on-time completion is greater than its parent graph, then we examine another iteration of partitioning. The stopping condition for partitioning is to reach graphs with only one vertex (one micro-service). 




==> Sources/relatedwork.tex <==
\section{Background and Prior Studies}\label{relatedwork}
Industry 4.0, has created the demand for micro-service-based applications that ensure the industrial sector’s efficiency, productivity, and safety.
Various research works (\cite{oluyisola2022designing,ammar2022implementing,laskar2022smart,al2022well,dai2022uav}) have been undertaken for the development and integration of smart applications into the industrial sectors.
%Consequently, developed smart micro-service applications need execution plans and load-balancing algorithms to complete successfully. 
In (\cite{xu2018dynamic}), Xu \etal use static resource allocation and dynamic service migration to balance the load across edge-to-cloud continuum depending on CPU, RAM, and bandwidth demands. Micro-services were assigned to fog nodes based on their category and request generation rates. While this work considers a hierarchical federation of computing platforms across edge-to-cloud, our research considers a horizontal federation using peer computing platforms (\ie fog systems) which is more viable in remote industrial areas.

% On a different note, in a security-related study effort\cite{abdel2021federated}, Abdel-Basset \etal find that cyber threats are caused by the vast size and complexity of industrial cyber-physical systems (ICPs). The authors designed a federated deep learning model for threat hunting against ICPs that resembles the network’s temporal data and geographical contexts. The concept is intended for the deployment of micro-services on appropriate edge servers and can maintain sufficient resource allocation. Accordingly, the findings revealed that user privacy could be preserved while the system’s efficiency is increased. 

In traditional operational systems of the industrial sector, the centralized cloud can only support legacy applications (\cite{alam2021cloud,shastry2022approaches}) with a considerable latency-tolerant nature. On the other hand, modern Industry 4.0 applications are latency-sensitive and need a dynamic execution platform to support (near) real-time response time. As such, Rao \etal in (\cite{rao2021eco}) proposed a dynamic runtime for smart industrial applications that utilize 5G technology with edge-cloud architecture. This work uses application-specific knowledge to map the micro-services into the execution platform. However, authors consider only the predefined critical path's latency and disregard other micro-services that could form a new the critical path if they are poorly allocated. Additionally, they consider utilizing cloud data centers to overcome the emergency and oversubscribed situations. In contrast, our proposed solution considers all the micro-services (including those not on a critical path) to complete the execution across the fog federation with respect to the application deadline. Similarly, Faticanti \etal (\cite{faticanti2020throughput}) analyze the throughput desires of the micro-service applications while perform offloading to other fog systems. They addressed resource allocation challenges for the fog-native applications, built on a containerized micro-service modules. Two cascading algorithms make up the entirety of their approach. The first one separates fog application components according to throughput, and the second one governs the application orchestration across geographically distributed data centers.  

As smart IoT-based solutions become widespread, there is a need to handle machine learning (ML) applications on the network’s edge. Existing machine learning inference methods assume a homogeneous underlying system, and do not account for distributed computing infrastructure. Recent breakthroughs in AutoML (\ie employing ML-based automation) (\cite{garouani2022amlbid}), however, provide solutions for lightweight ML via model compression, pruning, and quantization. A related research work (\cite{ishakian2018serving}) examines the suitability of using a serverless architecture for AI application workloads. The research work evaluates the performance of using serverless functions to classify images using deep learning models. The authors find that warm serverless function executions have acceptable latency. However, cold starts have significant overhead, which could pose a problem for adherence to SLAs that do not account for this bimodal latency distribution. Furthermore, serverless frameworks lack access to GPUs, and functions are stateless, meaning each execution can only use CPU resources and cannot rely on the serverless platform runtime to keep state between invocations to optimize performance. As a result, serverless solutions will need to accommodate more stateful workloads in the long run. To achieve performance comparable to current non-serverless platforms, a declarative way of describing workloads and their requirements will be necessary, such as specifying the minimum time to keep warm containers (\cite{kumari2022mitigating}) and access to GPUs (\cite{risco2021gpu}). In an associated field of study (\cite{zhang2021serverless}), Zhang \etal explore and propose a serverless framework for video analytics pipelines based on deep neural networks (DNNs), which fully leverages the collaborative potential of client-fog-cloud architecture. By effectively coordinating fog and cloud resources, they achieve cost-effective and highly accurate video analytics. The proposed system incorporates a human-in-the-loop design approach to continuously improve the performance of models. Moreover, it offers various functionalities for creating and deploying video applications, alleviating developers from time-consuming tasks related to resource management and system administration. However, this work is curated for video processing tasks and incorporates cloud computing that can generate latency in time-sensitive smart applications.


Patterson \etal (\cite{patterson2021hardware}) have addressed the need for having a specialized software-hardware system stack and a coordination mechanism to support edge-based applications. They propose a swarm coordination platform for the efficient and scalable execution of workflows of complicated tasks using cloud and edge resources. Their hardware-software system stack tries to bridge the gap between centralized and distributed coordination. Their suggested approach uses domain-specific languages (DSL) to enhance programmability, automatically mapping tasks to cloud and edge resources, and providing hardware acceleration fabrics for remote memory access and networking. However, they do not consider oversubscribed situations and latency constraint smart applications. In contrast, our work considers oversubscribed situation in remote areas where monolithic and micro-service applications coexist. %Thus, this work enables a smart and robust fog federation that is aware of the underlying software architecture of the receiving applications and the stochastic execution behaviour caused by the computing platform (\ie fog federation).



==> Sources/resourceAllocation.tex <==
\section{Resource Allocation Method across Serverless Fog Federation}\label{resourceAllocation} 
% Resource allocation occurs when the partitioning is completed with an optimum number of partitions. 
% The partitioning method returns the whole application as one part to the resource allocation module for a monolithic application that is considered a single micro-service workflow. 
% The resource allocation method can capture the uncertainty in requests' arrival and making the fog system resilient and serverless. 
The resource allocation module is in charge of allocating arriving requests---either in form of monolithic applications or partitioned micro-service workflows---across the local or the federated fog systems. The allocation is performed based on the notion of \textit{relevance} that is defined as a fog system that maximizes the likelihood of meeting the deadline (a.k.a. the \emph{probability of success}) for a given request. The probability of success for a single unit of execution (\ie a micro-service or a monolithic application) on a particular fog system depends on the \textit{end-to-end latency} distribution of that unit on that fog. 


The end-to-end latency is comprised of the communication and computation latencies.
%Furthermore, to minimize frequent application reassignment and compound delay, we have decided that the micro-service cannot be relocated once an assignment choice is made.
Each fog system uses historical computational and communication latency information of various micro-services across different fogs in the federation to generate the probability distributed functions (PDFs). In analogy, this is very much like routing tables (\cite{}) commonly used by the Internet routers. Two matrices are maintained at each gateway, namely, Estimated Task Computation (ETC) (\cite{diaz2011energy}), and Estimated Task Transfer (ETT) (\cite{hussain2019federated}). 
The PDF of computational latency for micro-service type $i$ on fog system $j$ is stored in entry $ETC(i,j)$ that is also used by the partitioning method, as noted in the previous section. Similarly, entry $ETT(i,j)$ maintains the communication latency PDF of transferring data for micro-service $i$ to fog $j$. We note that using these matrices makes the resource allocation method aware of the communication latencies, whereas,  partitioning method is less granular and only is aware of the computational latency. There are existing methods based on machine learning or other statistical approaches (\eg \cite{,}) to construct and regularly update $ETC$ and $EET$ matrices without any interference on the system functionality.

For partition $\omega$ with source node (micro-service) $i$, the resource allocation method computes its end-to-end latency distribution on fog $j$ via convolving $D_\omega$ (see Equation~\ref{eq:convolve}) and $ETT(i,j)$. The end-to-end latency distribution is then used in Equation~\ref{eq:prob} to calculate the probability of completing partition $\omega$ before its deadline. Once we know the chance of success on all adjacent fogs in the federating, the one that offers the highest probability of on-time completion is chosen as the assignment destination for $\omega$.  


It is noteworthy that the probability of completing $\omega$ on the fog originally receives it (a.k.a. local fog) does not include any communication latency. This means that, $\omega$ is assigned to an adjacent fog in the federation (a.k.a. remote fog), only if it offers a greater probability of on-time completion even after accounting for the communication latency. However, utilizing a remote fog in a remote industrial place implies environmental uncertainties, in addition to the communication and computation uncertainties, that can practically undermine the benefits of minor superiority in the probability of on-time completion. That is, the likelihood of on-time completion of $\omega$ remotely should be \textit{significantly} higher than the local one, so that it is worthwhile allocating it remotely.
To assess whether the difference between remote and local execution is significant, we propose to use the notion of confidence intervals (CI) of the underlying end-to-end completion time distributions. In particular, we check whether the CI of the end-to-end completion time distribution of the remote fog overlaps with the CI of the local one. If they do not overlap, it implies that the remote fog is offering a statistically and practically higher chance of success to $\omega$, otherwise it is not worthwhile allocating it remotely.

The pseudo-code provided in Algorithm~\ref{alg:ci} expresses the resource allocation method that each gateway utilizes to take advantage of the federated fog system. The method is called \emph{Maximum Probability (MR)} and is invoked for the set of partitioned micro-service workflows, denoted as $M$. % the micro-service partitions are separated for further processing.
Using the deadline of each micro-service partition $\omega \in M$, from Step 2---10 of the algorithm, the algorithm calculates the local and remote completion time distributions and its probability of success both locally and on the adjacent fog systems. 
Next, Step 11 sorts the calculated probabilities on remote fogs in the descending order. If the probability of success on the local fog is higher, then $\omega$ is assigned to the local fog. Otherwise, $\omega$ is assigned to a remote fog if the CI of its end-to-end latency distribution (denoted $E_g(\omega)$) does not overlap with the distribution of the local one (Step 14---17). Otherwise, the same procedure is performed for the rest of the neighboring fogs. If no non-overlap adjacent fog is found, then $\omega$ is assigned to the local fog (default assignment in Step 12).

\begin{algorithm}[!h]
	\SetAlgoLined\DontPrintSemicolon
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\SetKwFunction{algo}{algo}
	\SetKwFunction{proc}{Procedure}{}{}
	\SetKwFunction{main}{\textbf{TaskAssignment}}
	\Input{set of partitions $M$; $ETC$ and $ETT$ matrices; and set of the adjacent fogs $G$}
	\Output{chosen fog $g\in G$ to assign each partition $\omega \in M$}
	%SHOULD WE WRITE ABOUT distribution?
        %Separate each microservice partition $m_i$ from partition set $M$\;
        \ForEach{$\omega \in M$}{
        $E_r(\omega) \gets$ completion time distribution of $\omega$ on local fog\;
       $P_r(\omega) \gets$ probability of success on local fog \;
	\ForEach{$g \in G$} {
        $E_g(\omega) \gets$ end-to-end completion distribution of $\omega$ on fog $g$\;
	  $P_g(\omega) \gets$ probability of success on $g$ \;
          \If {$P_g(\omega) > P_r(\omega)$} {	%$/* uniqueness$ $dominates$ $on$ $duplicity */$
				      \small{add $P_g(\omega)$ to $F$, as a potential fog for assignment}\;
       	        	        }
       	}        	        
	sort $F$ in descending order\;
        consider local fog $r$ as default assignment for $\omega$ \;
	\ForEach{$P_g \in F$} {
	\If {CI $E_g(\omega)$ has no overlap with CI $E_r(\omega)$} {	
				      assign $\omega$ to fog $g$ \;
				      exit the loop\;   	
       	        	        }
       	}        	        
	}
\caption{Pseudo-code of the Maximum Probability (MR) resource allocation method}\label{alg:ci}
\end{algorithm}


==> Sources/results.tex <==
\section{Performance Evaluation}\label{result}

\subsection{Experimental Setup}
EdgeCloudSim (\cite{sonmez2017edgecloudsim}) is a discrete event simulator that we have used to develop the solution and then evaluate its performance. We simulate fog systems with eight processing nodes that process between 1500 and 2500 Million Instructions Per Second (MIPs) that represent the heterogeneity of fog systems across the federation. The synthesized fog federation is considered to be distributed across a two-dimensional plane. Hence, every fog has coordinates defined by the x and y-axis. Accordingly, each fog can have a maximum of four neighbours, and the federation is horizontally scalable.

\begin{table}[h!]
\centering
\scalebox{0.70}
{\begin{tabular}{l||l|l|l|l}

\textbf{Application} & \textbf{DNN Model} & \textbf{Input Type} & \textbf{Scope} & \textbf{Framework}\\ \hline \hline
\textit{Fire} & Customized Alexnet & Video Segment & \begin{tabular}[c]{@{}l@{}}Control \&\\ Monitoring\end{tabular} & \begin{tabular}[c]{@{}l@{}}Tensorflow \\ (tflearn)\end{tabular}\\ \hline
\textit{\begin{tabular}[c]{@{}l@{}}HAR\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Customized Sequential \\ Neural Network\end{tabular} & Motion sensors & \begin{tabular}[c]{@{}l@{}}Workers \\ Safety\end{tabular} & keras\\ \hline
\textit{Oil} & FCN-8 & SAR Images & \begin{tabular}[c]{@{}l@{}}Disaster \\ Management\end{tabular} & keras\\ \hline
\textit{\begin{tabular}[c]{@{}l@{}}AIE \end{tabular}} & \begin{tabular}[c]{@{}l@{}}Temporal Convolutional\\ Network\end{tabular} & Seismic Data & \begin{tabular}[c]{@{}l@{}}Seismic\\ Exploration\end{tabular} & PyTorch\\ 
\end{tabular}}
\caption{\small{ML-based applications used in many Industry 4.0 use cases, such as oil and gas, along with their neural network model, input data type, usage scope, and ML framework. The non-abbreviated application names in this table are: fire detection (Fire), human activity recognition (HAR), oil spill detection (Oil), and acoustic impedance estimation (AIE).}}
\label{table:apptype}
\end{table}


\begin{table}[h!]
\centering
\scalebox{0.75}
{\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{\textbf{Mean and Standard Deviation of Execution Times (ms) on AWS}} \\ \hline
\textbf{Application} & \textbf{\texttt{Mem. Opt.}} & \textbf{\texttt{ML Opt.}} & \textbf{\texttt{GPU}} & \textbf{\texttt{General}} & \textbf{\texttt{Compute Opt.}} \\ \hline
\textit{Fire} & \begin{tabular}[c]{@{}c@{}}$\mu$=1461.8\\ $\sigma$=457.3\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=1281.7\\ $\sigma$=387.93\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=1349.5\\ $\sigma$=418.9\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$ =1534.8\\ $\sigma$=494.7\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=1421.4\\ $\sigma$=441.8\end{tabular} \\ \hline
\textit{\begin{tabular}[c]{@{}c@{}}HAR\end{tabular}} & \begin{tabular}[c]{@{}c@{}}$\mu$=1.27\\ $\sigma$=0.082\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=0.66\\ $\sigma$=0.006\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=0.51\\ $\sigma$=0.006\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$ =1.17\\ $\sigma$=0.042\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=0.66\\ $\sigma$=0.003\end{tabular} \\ \hline
\textit{\begin{tabular}[c]{@{}c@{}}Oil\end{tabular}} & \begin{tabular}[c]{@{}c@{}}$\mu$=269.9\\ $\sigma$=1.01\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=218.8\\ $\sigma$=0.66\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=65.98\\ $\sigma$=0.47\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=667.1\\ $\sigma$=2.26\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=242.9\\ $\sigma$=0.68\end{tabular} \\ \hline
\textit{\begin{tabular}[c]{@{}c@{}}AIE\end{tabular}} & \begin{tabular}[c]{@{}c@{}}$\mu$=7.02\\ $\sigma$=0.02\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=6.41\\ $\sigma$=0.03\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=7.55\\ $\sigma$=0.04\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=9.35\\ $\sigma$=0.06\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mu$=7.95\\ $\sigma$=0.02\end{tabular} \\ \hline
\end{tabular}}
\caption{\small{The execution time mean ($\mu$), and standard deviation ($\sigma$) for various Industry 4.0 applications across different AWS machines types.}}
\label{tab:meanAWS}
\end{table}

As for the workload to evaluate our methods, we consider the context of remote Industry 4.0 for oil and gas (\cite{hussain2022iot}). We consider four ML-based workflow applications, namely, Fire detection ( \textit{Fire}), human activity recognition (\textit{HAR}), oil spill detection (\textit{Oil}), and acoustic impedance estimation (\textit{AIE}) (\cite{hussain2020analyzing}) and they are uniformly distributed within the workload. Hence, total number of applications in the workload are equally divided into the four Industry 4.0 applications.

While exploring the micro-service workflow architecture, as shown in Figure \ref{fig:workflowMicro}, we find that there are seven micro-services for fire detection application. Similarly, the number of micro-services for oil spill detection, human activity recognition, acoustic impedance estimation are five, four, and four sequential (single-core) micro-services, respectively. In Oil, the micro-services forming the workflow are data pre-processing, dark spot detection, feature extraction, classification, and segmentation micro-services. For AIE application, the micro-services are for data pre-processing, initial model develop, inversion, and acoustic impedance estimation. For HAR application we use data pre-processing, feature extraction, classification, and activity recognition micro-services. Other characteristics of these applications are presented in Table \ref{table:apptype}. We benchmarked these applications on AWS and identified their statistical distributions of their execution times (in terms of MIPS) that are presented in Table~\ref{tab:meanAWS}. %Therefore, we implement four Industry 4.0 applications where two of them (fire detection, oil spill detection) have five micro-services and other two (human activity recognition and acoustic impedance estimation) have four micro-services. 
For monolithic workload, we use the same set of applications, however, we treat them as one unit and do not partition them. One reason that we study monolithic applications in the experiment section is to abstract our analysis from the impact of workflows, and merely focus on the impact of the resource allocation methods across the federation.


% Additionally, for micro-service workflow applications, we consider each micro-service to belong to a specific type that corresponds to the service type we synthesized from our earlier work (\cite{hussain2020analyzing}). 
%F%or instance, data pre-processing, noise removal, feature extraction, classification, and object detection are five different types of micro-services that are commonly found in Industry 4.0 ML-based applications. Accordingly, we synthesize these five types of micro-services and utilize them in developing four different workflow applications as mentioned earlier. 


Upon arrival of a request to a gateway, the micro-services comprising the application are allocated distinct deadlines, as mentioned in our system model. According to reference (\cite{salehi2016stochastic}), an individual deadline comprises the time a micro-service arrives and the total delay that the micro-service can withstand in an end-to-end scenario. The delay in communication, which includes both up-link and down-link delays, can substantially affect the deadline. Accordingly, we consider the communication delay in the deadline calculation. For micro-service $i$, the deadline $m_i^d$ is defined as $m_i^d$ = $arr_i$+$E_i$+$\epsilon$+$d_C$ , where $arr_i$ is the arrival time of request, $E_i$ is the average micro-service execution time, $\epsilon$ is a constant value defined by the processing fog device (slack time), and $d_c$ is the mean communication delay. To produce the inter-arrival rate of the requests, we synthesized from real-world workload investigated by the Extreme Scale Systems Center (ESSC) at Oak Ridge National Laboratory (ORNL) (\cite{khemka2014utility,khemka2015utility}). In order to remove the impact of any randomness in the evaluations, we carry out every experiment a total of 30 times and subsequently estimate the mean and 95\% confidence interval. 



% To simulate heterogeneity, we perform each workload with a different number of micro-service or monolithic applications that reflect variation in oversubscription level.

\subsection{Baseline Workflow Partitioning Methods}
\emph{Min-Cut partitioning:} cutting graph $G$ partitions its vertices (micro-services) into two disjoint proper subsets. In a weighted graph, the cost of a cut is the sum of weights that are involved in the cut. Hence, the term ``minimum cut'' refers to a cut that is either minimal in terms of the number of edges that cross the cut (when the edges are not weighted) or minimal in terms of the weights of the edges that cross the cut (weighted). Min-cut is a widely-used method in the literature (\cite{lochbihler2022mechanized}), therefore, we use it as a baseline method via considering a unit weight for edges of a workflow graph. %Then, we utilize different resource allocation techniques for various performance evaluation experiments.

\emph{Least data transfer:} Within a workflow, output of a preceding micro-service serves as the input data for another micro-service. The ``Least data transfer'' partitioning method (\cite{use a citation if used previously}) considers the magnitude of data-transfer between micro-services as the weights of edges. Accordingly, this method traverse all the edges and cuts the workflow from the point where the transferred data is minimum. 

\subsection{Baseline Resource Allocation Methods}
\emph{Minimum Expected Completion Time (MECT):}
This is a popular resource allocation method~(\cite{mokhtari2023e2c,salehi2016stochastic}) that, for each request arriving to the gateway, it utilizes the ETC matrix to compute the mean expected completion time across different fog systems. The fog system with the minimum expected completion time is then chosen to handle the request.

\emph{Maximum Computation Certainty (MCC):}
MCC is another method used in the literature (\eg \cite{hussain2018robust}) for resource allocation. It makes use of the ETC matrix to calculate the difference between the request’s deadline and its mean completion time
(called certainty). Then, the task is assigned to the fog system that offers the highest certainty.

\subsection{Experimental Results}
% In the first experiment, the proposed partitioning method is compared against baseline methods to see how the deadline restrictions for workflow applications based on micro-services have improved. After partitioning, resource allocation to those partitions must be assessed. Hence, to evaluate the system's effectiveness, we conduct the second category of experiments that contrasts our suggested resource allocation strategies with alternative baselines. Then, we conduct the third experiment to see how scaling the fog federation affects the proposed solution. Finally, we analyze the computational latencies derived from partitioning and resource allocation methods for micro-service and monolithic applications. The following subsections provide a thorough description of the experiments.

\subsubsection{Evaluating the Impact of Workflow Partitioning}
To examine the impact of workflow partitioning, in this experiment, we study a scenario where no method for workflow partitioning is in place, therefore, the whole workflow is either executed locally or outsourced to another fog in the federation. We compare this scenario against cases where partitioning can be performed when needed using ProPart method. To further study the impact of partitioning, we compare the performance (ProPart) against other baseline methods for partitioning, namely Min-cut and Least data transfer. For the purpose of this experiment, we increase the number of workflow requests submitted to a gateway to generate oversubscribed conditions and record the rate of meeting deadline for each case. For this experiment, we configure Max Probability (MR) as the resource allocation method. The result of this experiment is shown in Figure \ref{fig:partitionComparison}. The horizontal axis indicates the number of workflow requests received and the vertical axis shows the rate at which application deadlines have been met.

\begin{figure}[h!]
	\centering	
	\includegraphics[scale=0.55]{Figures/WPartition_Comp_DeadlineMeet3.pdf}
	\caption{Comparison of the workflow partitioning methods. The horizontal axis represents the number of arriving workflow requests and the vertical axis shows the requests' deadline meeting rate.\label{fig:partitionComparison}}
\end{figure}  

The experiment results indicate that, in all cases, the percentage of workflows meeting their deadlines decline upon increase in the number of requests. Nonetheless, the advantages of workflow partitioning is significant, with ``No partition'' invariably performing poorly. We witness that partitioning can improve the performance of using federation by at least 5\% (``No Partition'' versus ``Least data transfer'' with 400 requests), and at most 35\% (``No Partition'' versus ``ProPart'' with 100 requests). Moreover, across various partitioning methods, we observe that ProPart surpasses other partitioning methods (particularly when the system is not oversubscribed), whereas, Least data transfer yields the lowest deadline meet rate. The reason for the higher performance of ProPart is that, under lower load, its statistical analysis to obtain the likelihood of success leads to more accurate results, thereby, more informed partitioning decisions. Moreover, we observe that, as the number of requests rises, the performance of Min-cut gradually drops to the extent that for 400 requests, it even gets marginally worse than the Least data transfer method. The reason is that, Least data transfer partitions based on the edges that generate the smallest output data that is effective when the system becomes oversubscribed, whereas, Min-cut utilizes the least number of edges for partitioning and does not consider the amount of data travels between the partitions. %Finally, due to the repeated probabilistic calculation of latency requirements for all micro-services, $ProPart$ performed better in totally oversubscribed conditions.

\subsubsection{Evaluating the Impact of Resource Allocation}
To study the impact of the resource allocation method in the fog federation, we performed the following experiments with three different resource allocation methods that, include the proposed MR method and two baseline methods, MECT and MCC. To studying the impact of using serverless federation fog versus not using it, we also include a scenario where no federation is utilized. We conducted this experiment for micro-service workflows, monolithic applications, mix application workload and the results are shown in Figures~\ref{fig:resourcAllocationComp} \ref{fig:resourcAllocationComp2}, and \ref{fig:mixWorkload} respectively.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{Figures/ResourceAlloc_Comp_Micro2.pdf}
    \caption{The deadline meet rates resulted from the MR, MCC, and MECT resource allocation methods of micro-service workflows across the fog federation.}
    \label{fig:resourcAllocationComp}
\end{figure}

\emph{Micro-service Workflow Applications:}  Similar to the previous experiment, the number of workflow requests is incremented to examine various levels of oversubscription, which is shown in the horizontal axis of Figure~\ref{fig:resourcAllocationComp}. In this experiment, we use ProPart to partition the micro-service applications. This implies that the MR bars, in the figure, show the performance of the entire methods we proposed in this work. To visualize the performance of the resource allocation methods, the deadline meet rates of receiving requests are reported. We can see that the benefits of making resource allocator aware of the fog federation is significant, because no federation scenario performed worse than the ``No Federation'' at any oversubscription level. This is because in a no-federation scenario, the recipient fog becomes overwhelmed with numerous requests, leading to missing request deadlines. Upon increasing oversubscription level, we can see a downward trend for all the resource allocation methods. However, because the proposed resource allocation method, MR, is aware of the compound uncertainty in both computation and communication, it still outperforms other baseline methods. In contrast, MECT and MCC are only cognizant of computation latency and the deadlines, therefore, they are prone to less informed allocation decisions that can cause missing the requests' deadlines. We can also observe that the performance difference of MCC and MECT is not statistically significant, because their confidence intervals overlap throughout the experiment. 

\emph{Monolithic Applications: } 
In this part, we investigate the performance of our resource allocation methods on the monolithic applications submitted to the system of fog federation. In addition we include a scenario where no federation is utilized to understand the benefits of using federated fog systems. In Figure \ref{fig:resourcAllocationComp2},  we can see the impact of increasing the number of incoming applications from 400 to 1,000 (horizontal axis) on the deadline meet rate (vertical axis) when various resource allocation heuristics are employed.
In fact, we performed the experiment for oversubscription levels less than 400, however, we did not observe any behavioral difference. As such, for the sake of better presentation, we only report results for cases where the number of requests are greater than 400.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{Figures/ResourceAlloc_Comp_Mono2.pdf}
    \caption{The deadline meet rate resulted from various resource allocation methods for monolithic applications across the fog federation.}
    \label{fig:resourcAllocationComp2}
\end{figure}

Similar to the previous case, in Figure \ref{fig:resourcAllocationComp2}, we observe the poor performance resulted by ignoring the federation. The issue becomes increasingly pronounced as oversubscription level rises (800 and 1,000 requests), highlighting the advantage of serverless fog federation for Industrial use cases in remote areas. With 1,000 requests, MR offers around 19\% higher deadline-meeting rates than the other two methods. The reason is that MR captures end-to-end latency and utilizes the federation only if it significantly impacts the chance of success. From these experiments, we can conclude that for both monolithic and workflow applications, capturing uncertainty of the end-to-end latency can significantly improve the performance. This impact is more remarkable for monolithic tasks, \ie monolithic tasks can make a better use of the federation, because they do not have the challenge of request partitioning and performing one request across multiple sites.

\emph{Mixed Application Workload:} To further evaluate the impact of resource allocation, in this experiment, we consider circumstances where the arriving workload is a mix of requests for monolithic and workflow applications. 50\% of the examined workload are requests for monolithic applications and another 50\% are micro-service workflows. Similar to the previous parts, we increase the number of requests (horizontal axis in Figure \ref{fig:mixWorkload}) and measure the deadline meet rate (vertical axis in the same figure). We use ProPart for partitioning the workflow applications along with various resource allocations methods.% For monolithic applications we use same resource allocation methods without partitioning method.
% The result of this experiment is presented in Figure \ref{fig:mixWorkload} where $x$ axis is defined as number of incoming application requests and $y$ axis is defined as deadline meet rates of the workload applications. 


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{Figures/proPart_mix_workload1.pdf}
    \caption{The deadline meet rate resulted from various resource allocation methods for mixed workload of monolithic and micro-service workflows across the fog federation.}
    \label{fig:mixWorkload}
\end{figure}

%The result in Figure \ref{fig:mixWorkload} present the benefit of utilizing our proposed partitioning method along with resource allocation method. Similar to previous results, we see a downward trend in every oversubscription level. Although, in every execution trial our proposed solution ($ProPart-MR$) outperform other baselines. For fully oversubscribed level (1000 requests) our solution performed better than only micro-service workflow application workload case and less than only monolithic application workload case. This average performance is because 50\% monolithic applications utilizes the federation effectively using $MR$ resource allocation method that proactively improve the chance of success for every monolithic request. In contrast, micro-service workflow application requests consider the partitioning method for more informed execution that reduce the performance. Even though our proposed solution for both type of applications outperforms other baselines due to utilizing end-to-end latency and serverless fog federation.

% Our methods for workflow partitioning and resource allocation have shown to be effective, as evidenced by the result shown in Figure \ref{fig:mixWorkload}. 
Decreasing the performance (deadline meet) upon increasing the number of requests aligns with our observations in the previous parts. However, we can see that even under mixed workload the combination of ProPart+MR consistently outperforms other methods for any level of request intensity. Although the performance difference of MR and other methods is not as significant as those in Figure~\ref{fig:resourcAllocationComp2} (for monolithic applications), it still outperforms the other methods due to the consideration of the end-to-end latency in the serverless fog federation. Analyzing other outputs of this experiment showed that, for monolithic requests, MR helped effective use of the federation and improving their performance, whereas, for micro-service workflow requests, the partitioning method contributes more than the resource allocation to the better performance.


\subsubsection{Analyzing the Workflow Makespan Time}
After scrutinizing behavior of the partitioning and resource allocation modules, in this part, our objective is to study the impact of entirety of the proposed solutions on the completion of requests. In fact, partitioning and and resource allocation methods can affect the computational latencies of the micro-service workflows. For the monolithic applications, resource allocation method is the influential factor on the requests' computational latencies. We measure the computational latency via the makespan time, which is the total processing time from the time a request is received until it is complete. Therefore, we capture the makespan time both for the micro-service and monolithic applications. We note that the experiments in the previous part only show the deadline meet rate and do not show how long on average all requests take to complete. 

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.58]
    {Figures/AvgMakespanTime_MicroPartition_Comp.pdf}
    \caption{Average makespan time for micro-service workflows utilizing various partitioning methods along with the MR resource allocation method}
   \label{fig:microMakespan}
\end{figure}

\emph{Average Makespan Time for Micro-service Workflows:}
In this part, we estimate the average makespan time of the workflow requests on the fog federation. Similar to the previous experiments, we increase the oversubscribing level by submitting more workflow requests. The result of this experiment is presented as a line chart in Figure~\ref{fig:microMakespan} where the x-axis represents the number of receiving requests, and the y-axis represents the average makespan time. We examine various partitioning methods and keep MR, as the resource allocation method. 

The general observation shows an upward trend in the average makespan time, regardless of the partitioning method. The difference across methods become visible after 200 requests. We can see that ProPart outperforms the other two baselines upon increasing the oversubscription level. This is because ProPart performs partitioning only if the success rate of completion is significant. On the other hand, the baseline methods partition requests without considering the latency constraints. %Therefore, $ProPart$ performed better than the baselines for highly oversubscribed situations.

\emph{Average Makespan Time for Monolithic Applications: }
Due to cohesion of monolithic applications, their computational latency is only influenced by the resource allocation method. Hence, we study the impact of various resource allocation methods on the makespan of the monolithic applications across the fog federation.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.58]
    {Figures/AvgMakespanTime_Monolithic3.pdf}
    \caption{Average makespan time resulted from various resource allocation methods for the monolithic applications}
    \label{fig:monoMakespan}
\end{figure}

The result of this experiment is presented in Figure~\ref{fig:monoMakespan}, demonstrating that MR and MECT perform similarly unless the system is highly oversubscribed. Moreover, MCC performs significantly worse for any workload size. The reason is that MCC do not consider the stochastic nature of completion time, hence, it assigns the arriving requests to one fog and oversubscribes that, which increases the average makespan. From the experiment, we can conclude that if the system is not oversubscribed, the serverless fog federation system does not need to undergo the complication of methods like MR and other methods like MECT and even MCC can provide a competitive performance. However, if the system is expected to receive higher amount of load, then methods that consider factors such as end-to-end latency are needed to better cope with the oversubscription.



\subsubsection{The Impact of Fog Federation Scaling}
The serverless fog federation in remote Industry 4.0 sites can potentially have a dynamic topology. For instance, when a disaster occurs in an offshore oil field, one or more rescue boats with mounted fog systems can be dispatched to seamlessly augment the existing fog and help in handling the disaster (\cite{gima2019model}). Conversely, in the event that one or more of these mobile fogs fail or leave the disaster place, a performance drop can potentially happen. The purpose of this experiment is to understand the impact of such dynamics on the overall fog federation performance. 

To achieve our goal, we insert neighbouring fog systems ranging from one to four that correspond to degree one to four in the underlying fog federation graph. This means that, we develop a grid-based fog federation that can have minimum of one neighbour fog and maximum of four neighbour fog. To evaluate the system's performance, we capture the deadline meet rate of the requests under various oversubscription levels ranging from 100 to 400 workflow requests. This experiment utilizes the proposed ProPart partitioning and MR resource allocation methods. The result of this experiment is presented in Figure \ref{fig:fedScaling}. In addition, we performed a similar experiment for monolithic applications, where we fixed the number of receiving tasks to 1,000 requests and incremented the fog federation degree for various resource allocation methods. The result for the monolithic applications is presented in Figure~\ref{fig:fedScalingMon}.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{Figures/FedDegree_Micro.pdf}
    \caption{Impact of scaling the serverless fog federation for proposed partitioning and resource allocation methods upon increasing the oversubscription level for micro-service workflows. The degree represents the number of neighbors each fog system has.}
    \label{fig:fedScaling}
\end{figure}

\emph{Impact of Federation Scaling on Workflows: }
Figure~\ref{fig:fedScaling} demonstrates the results for scaling the fog federation. We can see that, for any level of oversubscription, the largest federation (degree=4) excels. Importantly, considerable performance improvement is seen for the higher oversubscription level (300 and 400 workflows). On the other hand, for less overloaded cases, the performance improvement of scaling is marginal. Our analysis reveals that this is because ProPar attempts to put the entire workflow into one fog system, rather than partitioning and distributing them across the federation. For the higher levels of  oversubscription, however, the proposed method more often utilizes the fog federation to distribute workflow partitions. That is the reason we witness a more substantial improvement in under higher oversubscription levels.
 

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.55]{Figures/FederationDegree_Monolithic1.pdf}
    \caption{Impact of scaling the fog federation when different resource allocation methods are employed for monolithic applications. The ``degree'' shows the number of neighbors the source fog system has in the federation.}
    \label{fig:fedScalingMon}
\end{figure}

\emph{Impact of Federation Scaling  on Monolith Applications: }
In this experiment, we examine the resource allocation methods for monolithic applications while scaling the fog federation. As we can see in Figure \ref{fig:fedScalingMon}, the monolithic applications are positively impacted by the federation scaling. The result reflected a significant performance improvement when the federation scaled up from degree 1 to 2, regardless of the resource allocation method employed. Degree 1 describes a topology where there are only two fogs in the federation. That is why, none of the methods perform well. Even under such a tight resource availability, we can see that the MR method outperforms others. Nevertheless, for the higher degrees, MR performs approximately 15---18\% better than MECT and MCC. As mentioned earlier, the main reason behind superiority of MR is considering both the communication and computation latencies in its decision making. This particularly shows how the communication latencies can be decisive is such environments and that is why the and end-to-end latency has to be considered. 


==> Sources/systemModel.tex <==
\section{System Model}\label{sysModel}
% The main objective of this research is to support the computational need of Industry 4.0 applications by utilizing nearby fog systems in a serverless setup. As such, we consider a dynamically formed fog federation connected over high-capacity wireless links that provide the users with the illusion of accessing serverless infinite cloud-like resources and the ability to handle the surge load across peer fog systems seamlessly. Consequently, 
As shown in Figure~\ref{fig:sysModel}, the system model of the proposed serverless fog federation comprises: (1) A gateway in each fog system that receives arriving application requests and transparently allocates them across the federation by considering the communications and computing uncertainties, the application architecture, and its latency requirements. (2) A network of wireless gateways where each gateway $G_i$ represents a fog system that takes care of the coordination and data transfer with peer fogs across the federation. Each fog is an autonomous entity with its own resources and policies. %we have resource heterogeneity across fogs, thus, the applications have different execution times on various fog systems. 

In this research, we consider an oversubscribed situation in a fog that is defined as a situation where the the system cannot complete all the arriving requests within their deadlines. Each workflow application, denoted $\omega$, is a $DAG = (V,E)$, where the set of vertices $V = \{m_1, m_2,..., m_n \}$ denotes the micro-services, and edge $e(m_i,m_j) \in E$ represents the precedence between $m_i$ and $m_j$ micro-services. Each micro-service $m_i$ has a known slack (a.k.a. deadline and denoted $m_i^\delta$), which is the time duration within that the micro-service has to complete its execution. Furthermore, for each micro-service $m_i$, we assume to know the statistical distribution of its computational latency (denoted $m_i^d$) representing the possible execution times of that micro-service on that fog. Such a statistical distribution can be obtained from profiling the past execution times of the same micro-service on the same fog system (\cite{salehi2016stochastic,gentry2019robust}).
% across fog federation.


%We assume every smart application has a starting and ending micro-service that reflects the flow of action within the application. Therefore the smart applications can be considered as Directed Graph
% In a typical industrial operation scenario, various application (\eg monolithic, micro-service) requests arrive at the fog load balancer module with their deadline constraints, presented as step 1 in figure \ref{fig:sysModel}. 
% As opposed to the micro-service-based workflow, which has various individual deadlines for each micro-service, we assume that 
Monolithic applications have a  ``full cohesion", thus, a single deadline for the entire application. While partitioning in monolithic applications is infeasible, workflows have a ``loose cohesion'' and can be partitioned at the micro-service granularity (see Step 1 in Figure~\ref{fig:sysModel}). 
As shown in Step 2 of the same figure, for each arriving request for a certain application, the the fog gateway is responsible of creating the serverless illusion for the users by taking care of two actions: (\textbf{a}) optimally partitioning the workflow (\eg partitions \circled{P1} and \circled{P2} in Figure~\ref{fig:sysModel}); and (\textbf{b}) allocating resources to each partition via fog gateways (\eg $G1$, $G2$, and $G3$ in Figure~\ref{fig:sysModel}) across the federation. Finally, in Step 3, the serverless fog federation executes the applications and generates the results. 

\begin{figure}[h!]
	\centering	
	\includegraphics[scale=0.42]{Figures/sysModelJournal-Page-3.drawio (1).pdf}
	\caption{System model of the proposed solution to allocate micro-service workflow or monolithic applications across a federation of three fog systems. Step 1 shows different applications arriving to the gateway of their local fog system. Step 2 shows the internal mechanics of each gateway that includes a ``graph partitioning'' and a ``resource allocator'' modules. The former is in charge of transparently partitioning the micro-service workflows to maximize its likelihood of on-time completion. The latter is in charge of seamlessly allocating each partition to a fog across the federation. Step 3 shows the serverless fog federation where each fog is represented by a gateway ($G_1, G_2, G_3$).\label{fig:sysModel}}
\end{figure}

We assume the types of industrial applications operating in the system are limited and known in advance. Accordingly, the gateway stores and updates the computation and communication latencies of various categories of applications on the serverless fog systems. The computational latencies for various micro-services are captured in a matrix, termed as Estimated Task Completion (ETC) where each entry represents computational latencies for a particular micro-service across the fogs in the federation. Similarly, the communication latencies for various micro-services reaching various fog systems of the federation is stored in a matrix table and named as Estimated Task Transfer (ETT). The information from these two matrices are employed to estimate the applications' time constraints. That is, the gateway relies on this information to make informed decisions regarding resource allocation across the fog federation.



%Hence, partitioning is repetitive until the solution finds the optimum number of partitions. To be more specific, if further partitioning does not bring more likelihood of completion, then partitioning is not considered. Therefore, the proposed solution identifies the optimum number of partitions with a high chance of completion within the deadline constraints.


